Enhancing Navigational Safety in Crowded Environments using Semantic-Deep-Reinforcement-Learning-based Navigation

Intelligent navigation among social crowds is an essential aspect of mobile robotics for applications such as delivery, health care, or assistance. Deep Reinforcement Learning emerged as an alternative planning method to conservative approaches and promises more efficient and flexible navigation. However, in highly dynamic environments employing different kinds of obstacle classes, safe navigation still presents a grand challenge. In this paper, we propose a semantic Deep-reinforcement-learning-based navigation approach that teaches object-specific safety rules by considering high-level obstacle information. In particular, the agent learns object-specific behavior by contemplating the specific danger zones to enhance safety around vulnerable object classes. We tested the approach against a benchmark obstacle avoidance approach and found an increase in safety. Furthermore, we demonstrate that the agent could learn to navigate more safely by keeping an individual safety distance dependent on the semantic information.

==> ieeeconf/content/acknowledgment.tex <==
% !TeX encoding = utf-8
% !TeX language = en_GB
% !TeX spellcheck = en_GB
% !TeX root = paper.tex



==> ieeeconf/content/keywords.tex <==
% !TeX encoding = utf-8
% !TeX language = en_GB
% !TeX spellcheck = en_GB
% !TeX root = paper.tex


%\begin{IEEEkeywords}
%	Virtual Reality and Interfaces, Localization, Object Detection, Computer Vision for Other %Robotic Applications, AI-Based Methods
%\end{IEEEkeywords}

==> ieeeconf/content/rough_answers.tex <==
a. Necessity of Categorization of people into adult, child and elder people? How do you choose the classification ? How comes that ground truth in reality and simulation? how does the system collect semantic information in real world?

  Our task design is to adapt the behavior for different kinds of people (socially aware navigation), which demands the classification. The classifiaction is assumed to be obtained from the simulator of Pedsim during simulation. And in reality it should be detected directly by deep learning frameworks such as Detectron and Darknet. 
  
b. Justification of using both of the obstacle location and lidar scan:

The reason is that: lidar scan is used to supply the local map and coarse posistion of robot, and the precise location of humans are needed to encode the social interaction with robot. There are  two different body net for processing lidar scan and human states with robot states.

d. The semantic information is actually implicitly
encoded in the reward function with different sizes of
safety zone for different obstacle categories. One question
here: is the semantic input that helps the agent to learn a
safer navigation behavior or the more tough reward design
that considers the dynamic safety zone that does this?

The observation space depends on the reward system. The reward systems are designed with different sizes of safety zones depending on 
the categories of obstacles. So the agent should know the semantic info such as obstacle ID to form the logical relationships between the different safety sizes and the obstacle type. 


f.In comparison with the RAW laserscan baseline, do you utilize
the same reward function with the safety zone to assure a fair comparison ? 
Explained by Linh.




==> ieeeconf/content/title.tex <==
% !TeX encoding = utf-8
% !TeX language = en_GB
% !TeX spellcheck = en_GB
% !TeX root = paper.tex

%\title{A robust pose estimator for articualted robots using monocular cameras and Deep-Learning-based keypoint detection\\
%	}
%	\thanks{Identify applicable funding agency here. If none, delete this.}
%}
\title{\LARGE \bf
Towards Augmented Reality Simulation in Robotics - Facing Barriers of Industrial Applicability
}

\author{Jens Lambrecht$^{1}$, Linh Kästner$^{1}$, Jan Guhl$^{2}$ and J\"org Kr\"uger$^{2}$% <-this % stops a space% <-this % stops a space
% \thanks{*This work was not supported by any organization}% <-this % stops a space
\thanks{$^{1}$Jens Lambrecht and Linh Kästner are with the Chair Industry Grade Networks and Clouds, Faculty of Electrical Engineering and Computer Science,
        Technische Universität Berlin, 10587 Berlin, Germany
        {\tt\small lambrecht@tu-berlin.de}}%
\thanks{$^{2}$Jan Guhl and J\"org Kr\"uger are with the Chair Industrial Automation Technology, Faculty of Mechanical Engineering and Transport Systems,
        Technische Universität Berlin, 10587 Berlin, Germany
        {\tt\small guhl@iat.tu-berlin.de}}%        
}


%\author{
%	\IEEEauthorblockN{Jens Lambrecht}
%	\IEEEauthorblockA{\textit{Chair Industry Grade Networks and Clouds} \\
%		\textit{Technische Universität Berlin}\\
%		Berlin, Germany \\
%		lambrecht@tu-berlin.de}
%}

\maketitle
